Target-adaptive CNN-based pansharpening

We recently proposed a convolutional neural network (CNN) for remote sensing image pansharpening obtaining a significant performance gain over the state of the art. In this paper, we explore a number of architectural and training variations to this baseline, achieving further performance gains with a lightweight network which trains very fast. Leveraging on this latter property, we propose a target-adaptive usage modality which ensures a very good performance also in the presence of a mismatch w.r.t. the training set, and even across different sensors. The proposed method, published online as an off-the-shelf software tool, allows users to perform fast and high-quality CNN-based pansharpening of their own target images on general-purpose hardware.

==> tex - arXiv.R1.4/preambol.tex <==
% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


\usepackage{color,soul}
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{balance}
\usepackage{url}
\usepackage{multirow,hhline}
\usepackage{placeins}
\usepackage{wasysym}
\usepackage[nomessages]{fp}% http://ctan.org/pkg/fp



%%% PATHS
\newcommand{\tabPath}{./R1.tables/}
\newcommand{\figPath}{./R1.figures/}
\newcommand{\AdeImFolder}{\figPath samples_selected/Adelaide/}
\newcommand{\StockImFolder}{\figPath samples_selected/Stockholm/}
\newcommand{\WashImFolder}{\figPath samples_selected/Washington/}



% My commands
\renewcommand{\aa}[1]{{\bf \textcolor{blue}{#1}}}
\newcommand{\bb}[1]{{\bf \textcolor{red}{#1}}}
\newcommand{\point}{\item \vspace{-2mm}}
\newcommand{\Dlambda}{{\bf D}$_\lambda$}
\newcommand{\Desse}{{\bf D}$_S$}
\newcommand{\ru}{\rule{0mm}{3.2mm}}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\hx}{\widehat{\mathbf{x}}}

\newcommand{\M}{\mathbf{M}} % original res. MS
\newcommand{\PAN}{\mathbf{P}} % original res. PAN
\newcommand{\F}{\mathbf{F}} % original res. PANSHARPENED / FUSED
\newcommand{\R}{\mathbf{R}} % original res. REFERENCE
%\newcommand{\Mr}{\mathbf{\overline{M}}} % reduced res. MS
%\newcommand{\PANr}{\mathbf{\overline{P}}} % reduced res. PAN
%\newcommand{\Fr}{\mathbf{\overline{F}}} % reduced res. PANSHARPENED / FUSED
%\newcommand{\Rr}{\mathbf{\overline{R}}} % reduced res. REFERENCE



\DeclareMathOperator{\BN}{BN}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\Q}{Q}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\SAM}{SAM}
\DeclareMathOperator{\RMSE}{RMSE}
\DeclareMathOperator{\ERGAS}{ERGAS}
\DeclareMathOperator{\QNR}{QNR}
\DeclareMathOperator{\DS}{D_S}
\DeclareMathOperator{\DL}{D_{\lambda}}
\DeclareMathOperator{\DSast}{D_S^\ast}
\DeclareMathOperator{\DLast}{D_{\lambda}^\ast}




\newcommand{\rsize}[2]{
\FPeval{\result}{clip(#1*(#2-1)+1)}
\result$\times$\result
}

\newcommand{\nparam}[3]{
\FPeval{\result}{round(((#1-2)*(#2)*(#2)*(#3)*(#3) + 13*(#2)*(#3)*(#3))/10000,0)}
$\sim$\result$\cdot 10^4$
}

%\newcommand{\PNN}[3]{{PNN#1-F#2-#3$\times$#3}}
\newcommand{\PNN}[3]{{D#1-K#2-F#3}}

\newcommand{\p}{\noindent {\color{blue} $\RHD$ \rule{1mm}{0mm}}}

\newcommand{\image}{\pgfuseimage}



\pgfdeclareimage[width=0.95\columnwidth]{residuo}{\figPath residual.pdf}
\pgfdeclareimage[width=\columnwidth]{net}{\figPath net.pdf}

\pgfdeclareimage[width=0.9\columnwidth]{sam}{\figPath sam.pdf}
\pgfdeclareimage[width=0.9\columnwidth]{sid}{\figPath sid.pdf}
\pgfdeclareimage[width=0.9\columnwidth]{L2}{\figPath L2.pdf}
\pgfdeclareimage[width=0.9\columnwidth]{L1}{\figPath L1.pdf}
\pgfdeclareimage[width=\columnwidth]{Consistency}{\figPath Consistency.pdf}
\pgfdeclareimage[width=0.95\columnwidth]{up}{\figPath up.new.pdf}
\pgfdeclareimage[width=1.6\columnwidth]{finetune}{\figPath finetune.pdf}

% ISTOGRAMMI
\pgfdeclareimage[width=0.64\columnwidth]{Q_Caserta}{\figPath Q_Caserta.pdf}
\pgfdeclareimage[width=0.64\columnwidth]{Q_Ade}{\figPath Q_Ade.pdf}
\pgfdeclareimage[width=0.64\columnwidth]{Q_Wash}{\figPath Q_Wash.pdf}


% IMMAGINI TABELLA
\pgfdeclareimage{TabAde}{\tabPath WV3_Adelaide.pdf}
\pgfdeclareimage{TabStock}{\tabPath WV2_Stockholm.pdf}
\pgfdeclareimage{TabWash}{\tabPath WV2_Washington.pdf}
\pgfdeclareimage{TabWV}{\tabPath WV.pdf}
\pgfdeclareimage{TabGE}{\tabPath GE.pdf}
\pgfdeclareimage{TabIK}{\tabPath IK.pdf}

%\pgfdeclareimage{TabCplx}{\tabPath complexity.pdf}
\pgfdeclareimage{TabCplx}{\tabPath complexityFull.pdf}


% IMMAGINI DETTAGLI

\pgfdeclareimage{T6Stock}{\StockImFolder T6Stockholm.pdf}
\pgfdeclareimage{T5StockC}{\StockImFolder T5Stockholm_conf.pdf}
\pgfdeclareimage{T60Wash}{\WashImFolder T60Washington.pdf}
%\pgfdeclareimage{T3WashC}{\WashImFolder T3Washington_conf.pdf}
\pgfdeclareimage{T3WashC}{\WashImFolder T3Washington_conf_resized.pdf}
%\pgfdeclareimage{T20bAdeC}{\AdeImFolder T20bAdelaide_conf.pdf}
\pgfdeclareimage{T20bAdeC}{\AdeImFolder T20bAdelaide_conf_resized.pdf}



\definecolor{colPeppe}{rgb}{0.7, 0.2, 0.15}
\newcommand{\peppe}[1]{{\color{colPeppe} #1}}

\definecolor{colWarning}{rgb}{0.7, 0.2, 0.7}
\newcommand{\warning}[1]{{\color{colWarning} #1}}

\newcommand{\separatore}{\rule{0.9\columnwidth}{1pt}} 
